Channel Pruning for Accelerating Very Deep Neural Networks

In this paper, we introduce a new channel pruning method to accelerate very deep convolutional neural networks.Given a trained CNN model, we propose an iterative two-step algorithm to effectively prune each layer, by a LASSO regression based channel selection and least square reconstruction. We further generalize this algorithm to multi-layer and multi-branch cases. Our method reduces the accumulated error and enhance the compatibility with various architectures. Our pruned VGG-16 achieves the state-of-the-art results by 5x speed-up along with only 0.3% increase of error. More importantly, our method is able to accelerate modern networks like ResNet, Xception and suffers only 1.4%, 1.0% accuracy loss under 2x speed-up respectively, which is significant. Code has been made publicly available.

==> append.tex <==
\appendix
\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
	\hline 
	& $C1_1$ & $C1_2$ & $C2_1$ & $C2_2$ & $C3_1$ & $C3_2$ & $C3_3$ &$ C4_1$ & $C4_2$ & $C4_3 $ & $C5_1$ & $C5_2$ & $C5_3$\\ 
	\hline 
	channels & 64 & 64 & 64 & 128 & 128 & 256 & 256 & 256 & 512 & 512 & 512 & 512 &  512 \\ 
	\hline 
	filters      & 64 & 64 & 128 & 128 & 256 & 256 & 256 & 512 & 512 & 512 & 512 & 512 &  512 \\ 
	\hline 
	output size & 224 & 224 & 112 & 112 & 56 & 56& 56 & 28 & 28 & 28 & 14 & 14 &  14  \\ 
	\hline 
	Complexity(\%)& 0.6 & 12 & 6 & 12 & 6 & 12& 12 & 6 & 12 & 12 & 3 & 3 &  3  \\ 		
	\hline 
\end{tabular} 
\caption{VGG-16 Computational Complexity. Conv5 contributes little.}
\label{tab:vggcomp}
\end{table*}
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
	\hline 
	& $C1_1$ & $C1_2$ & $C2_1$ & $C2_2$ & $C3_1$ & $C3_2$ & $C3_3$ &$ C4_1$ & $C4_2$ & $C4_3 $ & $C5_1$ & $C5_2$ & $C5_3$ & 
	increase err.(\%)\\ 
	\hline 
	orig & 64 & 64 & 128 & 128 & 256 & 256 & 256 & 512 & 512 & 512 & 512 & 512 &  512 & 0(\origvgg) \\ 
	\hline 
	\x{2} & \eval{int(0.5*64)} & \eval{int(0.5*64)} & \eval{int(0.5*128)} & \eval{int(0.5*128)} & \eval{int(0.5*256)} & \eval{int(0.5*256)} & \eval{int(0.5*256)} & \eval{int(0.5*512)} & \eval{int(0.5*512)} & \eval{int(0.5*512)} & 512 & 512 &  512 & 0 \\ 
	\hline 
	\x{3.3} & \eval{int(0.25*64)} & \eval{int(0.25*64)} & \eval{int(0.125*128)} & \eval{int(0.125*128)} & \eval{int(0.25*256)} & \eval{int(0.25*256)} & \eval{int(0.25*256)} & \eval{int(0.25*512)} & \eval{int(0.25*512)} & \eval{int(0.25*512)} & 512 & 512 &  512 & \vggthreethree  \\ 		
	\hline 
	\x{4} & \eval{int(0.2*64)} & \eval{int(64)} & \eval{int(0.1*128)} & \eval{int(128)} & \eval{int(0.2*256)} & \eval{int(0.2*256)} & \eval{int(256)} & \eval{int(0.2*512)} & \eval{int(0.2*512)} & \eval{int(512)} & 512 & 512 &  512 & \vggfour \\
	\hline 
\end{tabular} 
\caption{Our reduction settings of \x{2}, \x{3.3}, \x{4} for vgg architecture. Shallower layers are heavily reduced.}
\label{tab:vgg}
\end{table*}
\begin{table*}
\centering
  \begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
 & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog  & horse  & mbike & person & plant & sheep & sofa &train  & tv & mAP \\ 
\hline 
original & 68.47 & 78.08 & 67.81 & 56.58 & 54.30 & 75.62 & 80.03 & 79.96 & 49.35 & 73.69 & 65.53 & 77.72 & 80.61 & 69.89 & 77.52 & 40.88 & 67.55 & 64.57 & 74.66 & 71.66 & 68.72  \\ 
\hline 
2x & 69.62&  79.33&  66.17&  56.09&  47.58&  76.79&  79.90&  78.18&  50.01&  72.98&  68.20&  75.74&  80.49&  74.81&  76.83&  39.12&  67.26&  66.76&  74.52&  66.13& 68.33 \\ 
\hline 
4x & 67.81 & 79.12 & 63.62 & 51.97 & 47.39 & 78.14 & 79.25 & 77.65 & 48.34 & 70.64 & 64.36 & 72.84 & 79.37 & 73.97 & 75.87 & 36.66 & 65.06 & 65.07 & 76.07 & 64.62 & 66.89 \\ 
\hline 
\end{tabular} 
\end{adjustbox}
\caption{details for faster RCNN detection acceleration}
\end{table*}
\begin{table*}[]
\centering
\begin{tabular}{|l|c|l|l|}
	\hline
	layer name & output size            &            kernel size, channels, stride               & computation       \\ \hline
	conv1      & 112$\times$112                & $7\times 7$, 64,stride 2 &    30\textperthousand              \\ \hline
	$2a_{1}$     & \multirow{4}{*}{$224/i^2\times224/i^2$} & $1\times 1$, 64,stride 2  & 13\textperthousand                 \\ \cline{1-1} \cline{3-4} 
	$2a_{2a}$    &                        & $1\times 1$, 64,stride 2  &   3\textperthousand           \\ \cline{1-1} \cline{3-4} 
	$ia_{1}$    &                        & $1\times 1$, 64,stride 2  &   26\textperthousand            \\ \cline{1-1} \cline{3-4} 
	$ia_{2a}$    &                        & $1\times 1$, 64,stride 2  &   6\textperthousand        \\ \cline{1-1} \cline{3-4} 
	$ix_{2a}$    &                        & $1\times 1$, 64           & 13\textperthousand   \\ \cline{1-1} \cline{3-4} 
	$ix_{2b}$    &                        & $3\times 3$, 64           & 29\textperthousand   \\ \cline{1-1} \cline{3-4} 
	$ix_{2c}$    &                        & $1\times 1$, 256          & 13\textperthousand  \\ \hline
\end{tabular}
	\caption{ResNet Computational Complexity}
	\label{tab:rescomp}
\end{table*}
